OptABC: an Optimal Hyperparameter Tuning Approach for Machine Learning Algorithms

Hyperparameter tuning in machine learning algorithms is a computationally challenging task due to the large-scale nature of the problem. In order to develop an efficient strategy for hyper-parameter tuning, one promising solution is to use swarm intelligence algorithms. Artificial Bee Colony (ABC) optimization lends itself as a promising and efficient optimization algorithm for this purpose. However, in some cases, ABC can suffer from a slow convergence rate or execution time due to the poor initial population of solutions and expensive objective functions. To address these concerns, a novel algorithm, OptABC, is proposed to help ABC algorithm in faster convergence toward a near-optimum solution. OptABC integrates artificial bee colony algorithm, K-Means clustering, greedy algorithm, and opposition-based learning strategy for tuning the hyper-parameters of different machine learning models. OptABC employs these techniques in an attempt to diversify the initial population, and hence enhance the convergence ability without significantly decreasing the accuracy. In order to validate the performance of the proposed method, we compare the results with previous state-of-the-art approaches. Experimental results demonstrate the effectiveness of the OptABC compared to existing approaches in the literature.

==> algorithm.tex <==
Algorithm \ref{alg:optABC} shows the previous work process\cite{zahedihyp}, along with the changes we made to improve the ABC convergence rate.
\begin{algorithm}
 \KwData{$Population\_number$, $Search\_Space$}
 %\KwResult{Cluster centroids}
 Call a function to create an initial population X{i} based on the hyper-parameters type and range\;
 Set the trail=0 for all food sources\;
 \While{Stopping criteria is not met}{
 \For {$i$ to $Population\_number$}{
  Employed bee generate a new food \(N{i}\) source in neighborhood and modify the new food source to an accepted food source \(M{i}\) (accepted type within range)\;
  \If { \(M{i}\) $==$ \(X{i}\) }{
  Move to step 5}
 
 Train the ML model with the modified food source\;
 \If { \(f(M{i})\) $<$ \(f(X{i})\) }{
  \(X{i}\) = \(M{i}\)\;
  Reset trial\;
  }
  \Else {Increment trial}
  }
  \For {$i$ to $Population\_number$}{
  \If { \((rand{(0,1)})\) $>$ \((P{i})\) }{
  Onlooker bee generate a new food source in neighborhood \(N{i}\) and then modify the new food source to an accepted food source \(M{i}\)
  
  \If { \(M{i}\) $==$ \(X{i}\) }{
  Move to step 16}
  Train the ML model with the updated food source\;
  \If { \(f(N{i})\) $<$ \(f(X{i})\) }{
  \(X{i}\) = \(M{i}\)\;
  Reset trial}
  \Else {Increment trial}
  }
  \Else {Onlooker disregard the food source and move to the next food source}
  }
  Memorize and update the best food source\;
  \If {trial $>$limit}{
  Scout bee generates a new random food source\;
  }}
 \Return Best found food source
 \caption{OptABC Algorithm}
 \label{alg:optABC}
\end{algorithm}


==> table.tex <==

\begin{table}[ht]
\centering
\caption{Performance evaluation of applying OptABC and HyP-ABC to the RF classifier on the MIDFIELD dataset.}
\label{tab:RF}
%\begin{adjustbox}{width=1.6\columnwidth,center}
\def\arraystretch{1.5}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{
  |c|c|c|c!{\vrule width 1.5pt} c|c|c|
  }
\hline
\multicolumn{7}{|c|}{\textbf{80:20 ratio Test-Train set}}\\
\hline
\textbf{} & \multicolumn{3}{c!{\vrule width 1.4pt}}{OptABC} & \multicolumn{3}{c|}{HyP-ABC}\\
\hline
\textbf{Population size} & \textbf{20} & \textbf{50} & \textbf{100} & \textbf{20} & \textbf{50} & \textbf{100} \\
\hline
\textbf{Accuracy(\%)} & 88.71 & 88.75 & 88.76 & 88.71 & 88.74 & 88.78\\
\hline
\textbf{\makecell{Execution Time(hrs)}} & 1.6 & 3.17 & 7.8 & 2.37 & 9.07 & 3.18\\
\hline
\multicolumn{7}{|c|}{\textbf{With 3-fold cross validation}}\\
\hline
\textbf{Accuracy(\%)} & 88.79 & 88.77 & 88.77 & 87.57 & 88.74 & 88.77\\
\hline
\textbf{\makecell{Execution Time(hrs)}} & 0.46 &  1.09 & 2.16 & \multicolumn{3}{|c|}{1.55 on average}\\
\hline
\end{tabular}
}
%\end{adjustbox}
\end{table} 

\begin{table}[ht]
\centering
\caption{Performance evaluation of applying OptABC and HyP-ABC to the XGBoost classifier on the MIDFIELD.}
\label{tab:XGB}
%\begin{adjustbox}{width=1.6\columnwidth,center}
\def\arraystretch{1.5}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{
  |c|c|c|c!{\vrule width 1.5pt} c|c|c|
  }
\hline
\multicolumn{7}{|c|}{\textbf{80:20 ratio Test-Train set}}\\
\hline
\textbf{} & \multicolumn{3}{c!{\vrule width 1.4pt}}{OptABC} & \multicolumn{3}{c|}{HyP-ABC}\\
\hline
\textbf{Population size} & \textbf{20} & \textbf{50} & \textbf{100} & \textbf{20} & \textbf{50} & \textbf{100} \\
\hline
\textbf{Accuracy(\%)} & 88.65 & 88.73 & 88.86 & 88.60 & 88.70 & 88.75\\
\hline
\textbf{\makecell{Execution Time(hrs)}} & 1.98 & 3.85&  3.42 & 4.07 & 5.85 & 4.23\\
\hline
\multicolumn{7}{|c|}{\textbf{With 3-fold cross validation}}\\
\hline
\textbf{Accuracy(\%)} & 88.29 & 88.64 & 88.72 & 87.97 & 88.64 & 88.84\\
\hline
\textbf{\makecell{Execution Time(hrs)}} & 4.83 &  19.54 & 17.6 & \multicolumn{3}{|c|}{29.22 on average}\\
\hline
\end{tabular}
}
%\end{adjustbox}
\end{table} 

\begin{table}[ht]
\centering
\caption{Performance evaluation of applying OptABC and HyP-ABC to the SVM classifier on the MIDFIELD dataset.}
\label{tab:SVM}
%\begin{adjustbox}{width=1.6\columnwidth,center}
\def\arraystretch{1.5}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{
  |c|c|c|c!{\vrule width 1.5pt} c|c|c|
  }
\hline
\multicolumn{7}{|c|}{\textbf{80:20 ratio Test-Train set}}\\
\hline
\textbf{} & \multicolumn{3}{c!{\vrule width 1.4pt}}{OptABC} & \multicolumn{3}{c|}{HyP-ABC}\\
\hline
\textbf{Population size} & \textbf{20} & \textbf{50} & \textbf{100} & \textbf{20} & \textbf{50} & \textbf{100} \\
\hline
\textbf{Accuracy(\%)} & 87.87 & 87.86 & 87.86 & 87.80 & 87.86 & 87.85 \\
\hline
\textbf{\makecell{Execution Time(hrs)}} & 18.3 & 8.61 & 15.5 & 23.95 & 53.05 & 62.57 \\
\hline
\multicolumn{7}{|c|}{\textbf{With 3-fold cross validation}} \\
\hline
\textbf{Accuracy(\%)} & 87.99 & 88.00 & 88.00 & 87.93 & 88.00 & 88.00 \\
\hline
\textbf{\makecell{Execution Time(hrs)}} & 19.71 &  39.01 & 40.10 & \multicolumn{3}{|c|}{34.15 on average} \\
\hline
\end{tabular}
}
%\end{adjustbox}
\end{table} 
